Managing Risk using Rolling Forecasts in Energy-Limited and Stochastic Energy Systems

We study risk-aware linear policy approximations for the optimal operation of an energy system with stochastic wind power, storage, and limited fuel. The resulting problem is a sequential decision-making problem with rolling forecasts. In addition to a risk-neutral objective, this paper formulates two risk-aware objectives that control the conditional value-at-risk of system cost and the buffered probability of exceeding a predefined threshold of unserved load. The resulting policy uses a parameter-modified cost function approximation that reduces the computational load compared to the direct inclusion of those risk measures in the problem objective. We demonstrate our method on a numerical case study.

==> Chapters/03_Risk-aware_decisions_with_Rolling_Forecasts.tex <==
\section{Risk-aware decision-making} \label{sec:risk-aware_decisions}
For any future $t'>t$, cost function \eqref{eq:cost_function} depends on uncertain system states $S_t(\omega)$ where $\omega\in\Omega$ is a random variable. To account for this uncertainty, decision-makers instead minimize expected cost $\mathbb{E}\big[\sum_{t'=t}^T(C_{t'}(S_{t'}(\omega), x_{t'}))\big],\ \forall t'$, e.g., as in \cite{Ghadimi2022}. 
This risk-neutral approach, however, is often not suitable for practical applications where decision-makers are risk-averse. This section briefly discusses options to handle risk. 


 
\subsection{Risk Measure: Conditional Value-at-Risk} 
\label{subsec:cvar}
Conditional Value-at-Risk ($\cvar$) is a popular risk metric in energy modelling due to its convex properties \cite{Stenclik2024}.
$\cvar$ is defined via the Value-at-Risk (VaR) $q_{\alpha}(X)$, which, for a given $\alpha \in [0,1]$, returns the minimum value $z$ that a random variable $X$ will not exceed with probability $\alpha$:
\begin{align}
    \var_{\alpha} (X):= q_{\alpha}(X) = \min \Big\{z \mid \mathbb{P}(X \leq d) \geq \alpha \Big\}. \label{eq:VaR}
\end{align}
VaR has useful applications for chance-constrained programs under some conditions, e.g., \cite{bienstock2014chance,lubin2015robust,mieth2019distribution}, but typically results in non-convex formulations.

$\cvar$ ($\bar{q}_{\alpha}$), on the other hand, captures the expected value of $X$ \textit{under the condition} that $X$ exceeds $q_{\alpha}$ \cite{Mafusalov2018}:
\begin{align}
  \cvar_{\alpha}(X) := \bar{q}_{\alpha}(X) = \mathbb{E} \Big[ X \mid X > q_{\alpha}(X) \Big]. \label{function:CVAR}
\end{align} 
For a linear cost function and assuming discrete outcomes (scenarios) $X_{\omega}$, $\cvar$ $\bar{q}_{\alpha}(X)$ can be minimized in a tractable linear program \cite{Mafusalov2018}:
\begin{subequations}
\begin{align}
    &\min_{x,z \in \mathbb{R},y_{\omega} \geq 0}
    && z + \frac{1}{1-\alpha } \sum_{\omega = 1}^{\Omega} \frac{1}{|\Omega|} y_{\omega}  \label{cvar_obj}  \\ 
    & \text{s.t.} && C(X_{\omega},x) - z - y_{\omega} \leq 0 & \forall \omega \in \Omega \label{cvar_const_1}.
\end{align}   
\label{eq:cvar_opt}
\end{subequations}

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth, keepaspectratio]{Pictures/CVaR_BPoE.pdf}
    \caption{Probability density function of a continuous random variable $X$. For a threshold $\zeta \in \mathbb{R}$, $p_x(X)$ equals $\mathbb{P}(X > z)$, which is the cumulative density (hashed area). For the same threshold $\zeta$, $\bar{p}_{\zeta}(X)$ is the cumulative density (solid+hashed area). The expectation of the worst-case $1 - \alpha = \bar{p}_{\zeta}(X)$ outcomes equals $\zeta = \bar{q}_{\alpha}(X)$.
    }
    \label{fig:CVAR_and_BPOE}
\end{figure}
Fig.~\ref{fig:CVAR_and_BPOE} illustrates the relation between $q_{\alpha}$ and $\bar{q}_\alpha$.
$\cvar$ allows to minimize the expected cost of the $100\alpha$-percent worst cases. In many engineering applications, however, risk-targets are not defined in terms of severity (probability times outcome), but whether a security threshold is maintained with high probability. 
We discuss this in the following section.


\subsection{Risk Measure: Buffered Probability-of-Exceedance} \label{subsec:bpoe}


Analogous to the relationship between VaR and $\cvar$, Buffered Probability-of-Exceedance ($\bpoe$) is defined via the Probability-of-Exceedance (PoE, or reliability), which
quantifies the probability mass of a random variable $X$ exceeding a given threshold $\zeta \in \mathbb{R}$ (see also Fig.~\ref{fig:CVAR_and_BPOE}):
\begin{align}
    \poe_{\zeta} := p_{\zeta}(X) = \mathbb{P}\Big[X > \zeta \Big].
\end{align}

PoE suffers the same mathematical shortcomings as VaR.
As the counterpart to $\cvar$ , $\bpoe$ overcomes these shortcomings and 
computes the risk-level $\alpha$ at which the $\cvar$ is equal to the predefined threshold $\zeta$ \cite{Mafusalov2018}:
\begin{align}
    \bar{p}_{\zeta}(X) = \underset{\gamma \geq 0}{\min} \quad \mathbb{E}\Big[\gamma ( X - \zeta) + 1 \Big]^{+},\label{eq:bpoe} 
\end{align} 
where $\gamma$ is an auxiliary variable and $[\cdot]^+ = \max\{\cdot, 0\}$.
Similarly to $\cvar$, minimizing $\bpoe$ over a set of scenarios $X_{\omega},\ \omega\in\Omega$ can be written as the linear program \cite{Mafusalov2018}:
\begin{subequations}
    \begin{align}
    &\underset{x, \gamma \geq 0 , \eta_{\omega} \geq 0}{\min} \ && 
    \sum_{\omega = 1}^{\Omega} \frac{1}{\Omega} \eta_{\omega} \label{bpoe_obj}  \\ 
    & \text{s.t.} && \gamma C(X_{\omega},x)\! - \!\gamma \zeta \!+\! 1\! -\! \eta_{\omega} \!\leq\! 0 & \forall \omega \in \!\Omega.  \label{bpoe_const}
    \end{align}%
    \label{bpoe_reformulation}%
\end{subequations}%
Term $\gamma C(X_{\omega},x)$ in \eqref{bpoe_const} allows the convex reformulation \cite{Mafusalov2018}:
\begin{equation}
    (C\gamma)(x) =  \begin{cases}
      \gamma C(x/\gamma) & \gamma > 0 \\
      0 &  \gamma = 0, x = 0 \\
      + \infty & \gamma = 0, x \neq 0.
    \end{cases}
\end{equation}

In contrast to $\cvar$, which has been connected to energy-based reliability metrics such as expected energy-not-served (EENS), e.g., in \cite{mieth2022risk}, the properties of $\bpoe$ allow to incorporate predefined frequency-based reliability metrics, e.g., the ``1 day in 10 years'' rule \cite{nerc2022Reexamining} or loss-of-load probability.
Hence, for a given $\zeta$
$\bpoe$ returns the probability that $C$ does not exceed $\zeta$ for a given decision $x$, thus \textit{certifying reliability.} 

